A determination of the fragmentation functions of pions, kaons, and protons with faithful uncertainties

We present NNFF1.0, a new determination of the fragmentation functions (FFs) of charged pions, charged kaons, and protons/antiprotons from an analysis of single-inclusive hadron production data in electron-positron annihilation. This determination, performed at leading, next-to-leading, and next-to-next-to-leading order in perturbative QCD, is based on the NNPDF methodology, a fitting framework designed to provide a statistically sound representation of FF uncertainties and to minimise any procedural bias. We discuss novel aspects of the methodology used in this analysis, namely an optimised parametrisation of FFs and a more efficient $\chi^2$ minimisation strategy, and validate the FF fitting procedure by means of closure tests. We then present the NNFF1.0 sets, and discuss their fit quality, their perturbative convergence, and their stability upon variations of the kinematic cuts and the fitted dataset. We find that the systematic inclusion of higher-order QCD corrections significantly improves the description of the data, especially in the small-$z$ region. We compare the NNFF1.0 sets to other recent sets of FFs, finding in general a reasonable agreement, but also important differences. Together with existing sets of unpolarised and polarised parton distribution functions (PDFs), FFs and PDFs are now available from a common fitting framework for the first time.

==> sec-pheno.tex <==

\section{Phenomenological implications at lepton and hadron colliders}
\label{sec:lhcpheno}

In this section we study the phenomenoligucal implications of the
NNFF1.0 set


\subsection{FCC-ee}

Compute fragmentation funciions ee

Check David, Peter

SIA

Check pheno implications


\subsection{LHC}

Here we use the same flavour separation as DSSZ

INCLNLO

Hannu


pPd AuAu
fragmentation



